Detecting out-of-context objects using contextual cues

This paper presents an approach to detect out-of-context (OOC) objects in an image. Given an image with a set of objects, our goal is to determine if an object is inconsistent with the scene context and detect the OOC object with a bounding box. In this work, we consider commonly explored contextual relations such as co-occurrence relations, the relative size of an object with respect to other objects, and the position of the object in the scene. We posit that contextual cues are useful to determine object labels for in-context objects and inconsistent context cues are detrimental to determining object labels for out-of-context objects. To realize this hypothesis, we propose a graph contextual reasoning network (GCRN) to detect OOC objects. GCRN consists of two separate graphs to predict object labels based on the contextual cues in the image: 1) a representation graph to learn object features based on the neighboring objects and 2) a context graph to explicitly capture contextual cues from the neighboring objects. GCRN explicitly captures the contextual cues to improve the detection of in-context objects and identify objects that violate contextual relations. In order to evaluate our approach, we create a large-scale dataset by adding OOC object instances to the COCO images. We also evaluate on recent OCD benchmark. Our results show that GCRN outperforms competitive baselines in detecting OOC objects and correctly detecting in-context objects.

==> tables/COCO-OOCaccuracy.tex <==

\begin{table}[t]
\caption{Accuracy score across OOC and non-OOC instances in our COCO-OOC and the OCD  dataset using oracle boxes. For OOC instances, \textbf{lower accuracy} is better and for non-OOC instances \textbf{higher} is better.}
\label{table:COCO-OOC-oracle}
\centering
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c}{Accuracy}  \\
  & OOC & non-OOC & Overall  \\
\midrule

GCRN (w/o ConG) & 0.69 & 0.77 & 0.76 \\
GCRN  & 0.30 & 0.98 & 0.93  \\
\bottomrule
\end{tabular}
\end{table}




